FAIRER: Fairness as Decision Rationale Alignment

Deep neural networks (DNNs) have made significant progress, but often suffer from fairness issues, as deep models typically show distinct accuracy differences among certain subgroups (e.g., males and females). Existing research addresses this critical issue by employing fairness-aware loss functions to constrain the last-layer outputs and directly regularize DNNs. Although the fairness of DNNs is improved, it is unclear how the trained network makes a fair prediction, which limits future fairness improvements. In this paper, we investigate fairness from the perspective of decision rationale and define the parameter parity score to characterize the fair decision process of networks by analyzing neuron influence in various subgroups. Extensive empirical studies show that the unfair issue could arise from the unaligned decision rationales of subgroups. Existing fairness regularization terms fail to achieve decision rationale alignment because they only constrain last-layer outputs while ignoring intermediate neuron alignment. To address the issue, we formulate the fairness as a new task, i.e., decision rationale alignment that requires DNNs' neurons to have consistent responses on subgroups at both intermediate processes and the final prediction. To make this idea practical during optimization, we relax the naive objective function and propose gradient-guided parity alignment, which encourages gradient-weighted consistency of neurons across subgroups. Extensive experiments on a variety of datasets show that our method can significantly enhance fairness while sustaining a high level of accuracy and outperforming other approaches by a wide margin.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/introduction.tex <==
\section{Introduction}
% introduction的逻辑跟abstract不一样，感觉为啥要去分析决策过程没讲清楚，
In current society, there is a desperate eagerness for social fairness among individuals. 
%
However, as deep learning is increasingly adopted for many applications that have brought convenience to our daily lives~\citep{ad,ab,as}, DNNs are still suffering from the fairness problem and often exhibit undesirable behaviors (\eg, discrimination) \citep{biasnews, ibmabandon}. For example, for an intelligent task (\eg, face expression classification), a trained DNN easily presents distinct accuracy values in different sub-groups (\eg, male and female).
%
The discriminatory behaviors contradict people's growing demand for fairness, which would cause severe social consequences. To alleviate such fairness problems, a line of mitigation strategies have been constantly proposed~\citep{f1,f2,f3}.

A direct regularization method to improve fairness is to relax fairness metrics as constraints in the training process~\citep{Madras2018LearningAF}. This regularization method is designed to reduce the disparities between different subgroups in the training and testing data. 
%
Although this method easily improves the fairness of DNN models, it is still unclear how the trained network makes a fair decision. For example, we do not know \textit{how the fairness regularization terms actually affect the final network parameters and let them make a fair prediction.} 
%
Without such an understanding, we may not know the effective direction for further fairness enhancement.
%
Existing works do not pay attention to this question and most of them mainly focus on the last-layer outputs (\ie, predictions) while neglecting the internal process.
%
In this work, we propose to study the fairness from the perspective of decision rationale and analyze existing fairness-regularized methods through a \textit{decision-rationale-aware analysis} method. 
%
The term `decision rationale' is known as the reason to make a decision and could be represented as the behaviors of neurons in a DNN \cite{Khakzar2021ICLR}.
%
Specifically, for each intermediate neuron (\ie, a parameter of the DNN),  we can calculate the loss change on a subgroup before and after removing the neuron.
%
As a result, we can characterize the decision rationale of a network on the subgroup by collecting the loss changes of all neurons.
%
Then, we define the \textit{parameter parity score} as the variation of the decision rationales on different subgroups, which actually reveals the influences of intermediate neurons (\ie, parameters) to the decision rationale changes.
%
With the new analysis tool, we find that the network's fairness is directly related to the consistency of the decision rationales on different subgroups and existing fairness regularization terms could partially achieve this goal since they only add constraints to the final outputs.
%
Intuitively, we could define new regularization terms to minimize parity scores of all neurons and encourage them to have similar behaviors across subgroups.
%
We name this new task as the \textit{decision rationale alignment} that requires DNNs to have consistent decision rationales as well as final predictions on different subgroups.
%
Although straightforward, the task is challenging due to two reasons: \textit{First}, the decision rationale and parity score are defined based on a dataset and it is impractical to calculate them at each iteration during the training process. \textit{Second}, different neurons have different effects on the fairness and such differences should be carefully considered.

To address the above two challenges, we propose the \textit{gradient-guided parity alignment} method by relaxing the calculation of decision rationale from the dataset-based strategy to the sample-based one. As a result, the corresponding regularization term is compatible with the epoch-based training process. Moreover, we use the first-order Taylor expansion to approximate the parity score between decision rationales, and the effects of different neurons on the fairness are weighted via their gradient magnitudes automatically. Overall, the proposed method is able to achieve much higher fairness than state-of-the-art methods.
%
% Note that, our main idea is similar with the human society where people are not only focusing on the \textit{outcome justice}~\citep{oj} (\eg, fairness in the decision results) but pay increasing attention to the \textit{procedural justice}~\citep{pj} (\eg fairness in the decision rationale). The regularization method to improve fairness can be deemed as achieving the \textit{outcome justice} directly. In this paper, our experiments/analysis show that \textit{procedural justice} might be easily violated in DNN models, which enlarges the trade-off between fairness and classification accuracy. We propose decision rationale alignment to further achieve the \textit{procedural justice} to minimize the trade-off.
%
In summary, the work makes the following contributions:
\begin{enumerate}
    %
    \item To understand how a network makes a fair decision, we define \textit{parameter parity score} to characterize the decision rationales of the network on different subgroups. We reveal that the fairness of a network is directly related to the consistency of its decision rationales on different subgroups and existing regularization terms cannot achieve this goal.
    %
    \item To train a fairer network, we formulate the \textit{decision rationale alignment} task and propose the \textit{gradient-guided parity alignment} method to solve it by addressing the challenges of the complex optimization.
    %
     \item Extensive experiments on three public datasets, \ie, Adult, CelebA, and COMPAS, demonstrate that our method is able to enhance the fairness of DNNs effectively and outperforms others largely.
    %\item We propose to understand the model decision rationale from the perspective of pruning in the spirit of decomposing DNNs. We calculate neuron importance to characterize and analyze the model decision rationale.
   

\end{enumerate}

%\litl{Specifically, if the decision results are still fair after decomposing the model to a sub-architecture model by removing any portion of neurons, the decision rationale of the model must be fair. However, the computation cost is too huge to optimize the model to assure the fairness of every sub-architecture. To address this issue, in our paper, we propose to directly compute the neuron importance to characterize the decision rationale for a group of data. We then approximate the alignment of decision rationales as the alignment of the neuron importance for different subgroups. The optimization target to ensure fairness for each sub-architecture could be relaxed into aligning the neuron importance of different subgroups on the current model, which avoids the actual decomposing process. Meanwhile, due to the fact that not all neurons contribute positively to the model classification, aligning the importance of all neurons might "distract" the model from aligning the "true" decision rationales (\ie, the neurons contribute significantly to the final classification). Therefore, this paper proposes the \tool method, in which we take an adaptive strategy to effectively and precisely align the importance of neurons contributing significantly and directly prune the redundant and less important neurons.} 


%we try to analyze the importance of each neuron to decompose the DNNs to characterize the decision rationale. Correspondingly, we then propose to approximate the alignment of decision rationales as the alignment of the neuron importance for different subgroups. Significantly, not all neurons contribute positively to the model classification. To remove the impacts of redundant neurons and precisely align the importance of neurons with large contributions, we take an adaptive strategy to prune the less important neurons.
% For a fair model, we expect that two subgroups of data are under the same decision rationale to assure {Procedural Justice}, which is further approximated as that two subgroups share the same important neurons. 
%Based on the above motivation, this paper propose the \tool method to approximate the alignment of decision rationale by selectively aligning the  neuron importance. 
%Nevertheless, we humans cannot easily understand the decision rationalees of deep learning models. The black-box nature of deep learning models restricts us to explicitly repair and align the decision rationalees for different subgroups. Fortunately, many approaches have been proposed to interpret the behaviors of deep learning models. A series of works[] focus on understanding the knowledge captured by DNNs and show the knowledge to humans in an understandable manner. Specifically, ~\cite{i1} designs a visualization method to comprehend the concept captured by a single neuron. Moreover, there are some recent works ~\cite{pr, npc} decomposing DNNs according to their semantics or functions. The layer-wise dataflow analysis is similar to the execution path of a control-flow based program~\cite{code}. Regarding individual neuron as a functional and semantic unit, such works analyze neurons which are mostly relevant to the final classification and select important neurons to depict the decision rationale of DNNs. Our work also follows the same thought, characterizing the decision rationale from the perspective of neuron importance analysis, which can be further formulated as a structural pruning problem. For a group of data, the neurons preserved after a round of pruning are critical to the classification for this subgroup. The preserved neurons could then be used to characterize the decision rationale of the model. For a fair model, we expect that two subgroups of data are under the same decision rationale to assure \textbf{Procedural Justice}, which is further approximated as that two subgroups share the same important neurons. We can also understand the approximation to the alignment of decision rationale from the point of neuron function: if each neuron plays an equal role in the decision of two subgroups, the discriminatory semantic information in neuron would be non-critical to the final decision of the model.

% More importantly, we find that when \textbf{Procedural Justice} is also satisfied besides \textbf{Entity Justice}, the trade-off between accuracy and fairness will be reduced. \todo{Meanwhile, as proposed in~\cite{overfitting}, the fairness constraints easily suffer from overfitting, \ie, \textbf{Entity Justice} and \textbf{Procedural Justice} are both satisfied on the training data but not fulfilled on the test data. Based on the aligned neuron importance, we can further do a unbiased structural pruning method to mitigate the overfitting. Significantly, in this paper, the aim of \textbf{Neuron Importance Alignment} is to further constrain \textbf{Procedural Justice} to ensure the authentic fairness on the training data to reduce the trade-off. The aligned pruning is designed to prevent overfitting to minimize the fairness discrepancy between the training data and the test data.} 







==> sections/methodology.tex <==
% \section{Selective Neuron Importance Alignment for Fairness}
\section{Methodology}
% In this paper, we propose to achieve \task between different subgroups in the spirit of decomposing DNNs.
In this section, we introduce our method to characterize the decision rationale of DNNs for each subgroup to avoid the heavy calculation of neuron discrimination; then, we introduce the decision rationale discrimination and provide our Neuron Importance Alignment approach to mitigate the decision rationale discrimination.

\subsection{Motivation}


% Based on the observation that ResAlign could ensure fair decision results to some extent while suffering from more severe trade-off~\cite{fairmixup, Du2021FairnessVR}, we hypothesize that the rationales behind the fair decision results are not consistent and the unfair decision rationale is a cause of the more severe trade-off. 

As shown in Figure \ref{fig:path}, the model trained by ERM exhibits a large divergence between the prediction accuracies of females and males. Although training by ResAlign successfully decreases the accuracy divergence, the overall prediction accuracy is severely compromised. To verify our hypothesis that the decision rationale of ResAlign is still unfair, we need to decompose the DNN to calculate $\mathbf{Gap}$ for all neurons according to Equation~\ref{equa:def2}. 

To avoid the huge computation cost, we propose a characterization method to depict the decision rationale. Via the characterization method which is based on neuron importance, we can easily analyze the divergence between the decision rationales of different subgroups. Furthermore, we propose to align the neuron importance to achieve decision rationale fairness.

\begin{figure*}
    \centering
    % \includegraphics[width=1\linewidth]{pics/overview.pdf}
    % edit link https://docs.google.com/drawings/d/18RlL7kaLESNMWN_KbEnKI62wJ4sB4gURKpqimwe2LkQ/edit?usp=sharing
    \includegraphics[width=1.0\linewidth]{pics/blue.pdf}
    \caption{The comparison of \tool with the baseline methods. The red line connects neurons critical for classification of subgroup "females". The blue line connects neurons critical for classification of subgroup "males". The grey line connects neurons critical before decomposition while non-critical after decomposition. The classification of models trained by ERM is biased. If the model is decomposed, the bias is even deteriorated. The models trained by ResAlign exhibit fair results while the decision rationales are different. The fairness should be destroyed when decomposing the model because the decision rationales are not consistent. Our method \tool 
   achieves the consistent decision rationales behind different subgroups through pruning redundant neurons and aligning the importance of neurons. \tool better reduces the trade-off. Significantly, our method enables us to calculate neuron importance to estimate the impact of "decompose", which avoids the time overhead needed in real pruning process.}
    \label{fig:path}
    % \vspace{-0.2in}
\end{figure*}

\subsection{Neuron importance Alignment}
\label{sec：cha}

% We expect to analyze the decision rationale of the model by estimating the Formula~\ref{equa:def} on the training data. However, a

\textbf{Characterizing Decision Rationale.} To bypass the huge calculating cost in Equation~\ref{equa:def2}, we propose to first characterize the decision rationale of each subgroup respectively via neuron importance estimation, which largely eases the computation and enables us to align the characterizations to achieve \taskns. In our paper, the neuron importance estimation method follows the calculation method proposed in~\cite{8953464}. Different from their work, we do a subgroup-wise estimation to characterize the decision rationale for each subgroup.


% The importance estimation follows the spirit of decomposing DNNs from the perspective of structural pruning.
% Fortunately, there are a series of work (\cite{goh2021multimodal}) exploring the DNN behaviors via neuron semantic analysis. 
Specifically, to estimate the importance $\mathbf{I}_m^{a,t,l}$ of neuron $m$ on layer $l$ of model $F$ for a group of data with sensitive attribute $a$ and label $t$, we calculate the squared difference of the loss when pruning the neuron $m$. 


% It is even harder to optimize the constraint for the model to minimize the influence gap of all neurons:
% \begin{equation}
% \begin{aligned}
% \min\sum_l^L\sum_{m\in F_l} \mathbf{Gap}_m^{l}.
% \end{aligned}
% \end{equation}

% Assuming that the constraint $\Delta EO$ is satisfied,
% % From the perspective of pruning, if a structural portion of the neurons is removed while the classification performance is rarely affected, the removed neurons are less important. 
% % The main information is propagated via these important neurons, which could depict the decision process of the model.
% we can modify $\mathbf{Gap}_m^{l}$ as follows:


% To reduce the computation cost, we approximate the calculation by its first-order Taylor expansion:

% \begin{equation}
% \begin{split}
% % \label{equa:D}
% \mathbf{Gap}_m^{l} = &\sum_{t \in \{0, 1\}} (|g_m^0 w_m| - |g_m^1 w_m|) ^2
% \end{split}
% \end{equation}


\begin{equation}
\label{equa:I}
\mathbf{I}_m^{a,t,l} = (E_{x \sim P_a^t}F(x) - E_{x \sim P_a^t}F(x, \mathbf{W}|w_m^l=0))^2.
\end{equation}

Using the first-order Taylor expansion, the estimation can be simplified to:

\begin{equation}
\label{equa:I}
\mathbf{I}_m^{a,t,l} = (g_m^{a,t,l} w_m^l)^2.
\end{equation}
where $g_m^{a,l}$ is the gradient of neuron $m$ when calculated on a subgroup of data. 
% Specially, for a group of data with sensitive attribute $a$, the neuron importance $\mathbf{I}_m^a$ could be represented by the error induced by removing the neuron $m$ in layer $l$:

Then the neuron importance of the layer $l$ composed of $M_l$ neurons could be represented as $\mathbf{I}^{a,t, l} = \{\mathbf{I}_0^{a,t,l}, \mathbf{I}_1^{a,t, l}, ..., \mathbf{I}_{M_l}^{a,t, l}\}$. We can further depict the neuron importance of the model $F$ as $\mathbf{I}^{a,t} = \{\mathbf{I}^{a,t, 0}, \mathbf{I}^{a,t. 1}, ..., \mathbf{I}^{a,t, L}\}$. Regarding individual neuron as function unit, $\mathbf{I}^{a,t}$ could reflect how these neurons' functions contribute to the final classification and then could be used to characterize the decision rationale for the subgroup of data with sensitive attribute $a$ and label $t$.

% In this way, the essence of a fair decision process is converted into neuron importance alignment for different subgroups. 

% \subsubsection{Analysis of Decision Results Fairness}


% \subsubsection{Fair Decision Process and Fair Output}

% In the next section, we will reveal that directly optimizing $\Delta DP$ and $\Delta EO$ does not guarantee a fair decision process, which causes a greater trade-off between accuracy and fairness. 

% For a group of data, we calculate the importance value $I$ for each neuron.
% If a portion of neurons in a model are disproportionately activated by different subgroups, this means these neurons exhibit distinguishing behaviors to different subgroups. In other words, the decision process for different groups differs and relies on sensitive information.

% However, if such neurons are important to the final model decision, the model would also exhibit distinguishing behaviors to certain subgroups.
% For a fair classifier, we expect the decision process barely rely on sensitive information. In other words, for neurons exhibiting distinguishing behaviors, 
% We expect these neurons to be less important to the final classification. 
% From the perspective of structural pruning, this could be transformed into when we prune neurons of the model, the impacts to different subgroups are similar. 
% We expect that, for a fair model, the neuron importance should satisfy $\mathbf{I}^0 = \mathbf{I}^1$.
% \subsection{Selective Neuron Importance Alignment Method}

% \subsubsection{Adaptive Neuron Importance Alignment}
 
% With the regularization to the fairness metrics $\Delta DP$ ~\ref{equa:DP}, the formula can be rewritten as:
% \begin{equation}
% \begin{aligned}
% \min\mathbf{Gap}_m^{a,l} &=|E(\mathbf{D}_{0}, \mathbf{W}) - E(\mathbf{D}_{0}, \mathbf{W}|w_m^l=0)| - |E(\mathbf{D}_{1}, \mathbf{W}) - E(\mathbf{D}_{1}, \mathbf{W}|w_m^l=0)|.
% \end{aligned}
% \end{equation}
% \subsubsection{Exploration of the Method ResAlign}


% As we mentioned above, the method \textbf{ResAlign} achieves the fairness in decision results while suffering from severe trade-off.
\textbf{Decision Rationale Discrimination.} To intuitively compare the decision rationale, we calculate $\mathbf{I}^{a,t}$ for each subgroup $\mathbf{g}_{a,t}$, $a,t \in \{0,1\}$ and we select layer-wise important neurons (\eg neurons with top importance in each layer) for observation. We could observe a clear correlation between the fairness metrics and the divergence between the important neurons for different subgroups.

For more elaborate analysis, we propose a metric to evaluate the similarity between neuron importance of different subgroups:
\begin{equation}
\label{equa:D}
S^l = cosine(\mathbf{I}^{0, l}, \mathbf{I}^{1, l})
\end{equation}
where $S^l$ is the neuron importance similarity in layer $l$ and $cosine(v1, v2)$ is a function to calculate the cosine similarity between $v1$ and $v2$. For smaller divergence between the decision rationales, it is desirable to have $S^l$ closer to 1.

% We examine the divergence of decision rationales between different subgroups. 
% can reveal that although the fairness between decision results is satisfied, there might be a large divergence between their decision rationales as shown in Figure \ref{fig:path}. This direct regularization achieves spurious decision results fairness on the training data while more discriminatory behaviors could still be easily triggered in the test data. To reveal the divergence, we propose to select neurons with top importance for analysis.



% \textbf{Individual Neuron Function Analysis.}
% \todo{
% We design methods to check the activation pattern of most important neurons for the training data. Firstly, we estimate samples that can obviously activate the most important neurons to check whether their activation patterns are biased.
% Secondly, we take grad-cam to visualize the activation region of the neuron to check whether these neurons are biased.}
Based on the analysis of top important neurons and the similarity $S^l$, we reveal that the decision rationale is not fair when trained by ResAlign. Also, we empirically show that the unfair rationale is a cause of severe trade-off (corresponding experimental results are in section \ref{sec:dra}). We conclude that only guaranteeing \textit{Outcome Justice} might result in superficial fairness on the training data. We propose to further ensure the \textit{Procedural Justice} to reduce the trade-off. 

\textbf{Model Repair via Neuron importance Alignment.}
We propose to align the neuron importance for \taskns. We formulate the optimization target as:

\begin{equation}
\label{equa:D}
\max\sum_{l}^LS^l =  \max\sum_l^L{cosine(\mathbf{I}^{0, l}, \mathbf{I}^{1, l})}.
\end{equation}

Combined with the constraint to ensure the decision results fairness, the final loss of our neuron importance alignment method is:
\begin{equation}
\label{equa:D}
\min\mathcal{L_{\text{\tool}}} = \min E_{x \sim P}F(x) + \lambda_1 \Delta EO - \lambda_2\sum_{l}^LS^l.
\end{equation}

As shown in Figure \ref{fig:path}, in the training process, we align the neuron importance which can avoid plausible biased decomposition, \ie, ensure the \taskns.

% 感觉应该注释掉，或者只截一个小片段
% \begin{wrapfigure}{R}{0.5\textwidth}
% \begin{minipage}{0.45\textwidth}
%   \begin{algorithm}[H]
%   \LinesNumberedHidden
%   \label{alg:alg}
%     \caption{Adaptive Neuron Importance Alignment}
%     \KwData{training epochs $e$, minibatch size $ms$, pruning threshold $pt$, max amount of prune neurons $pnm$, pruning frequency $pf$, pruning amount per minibatch $ppi$}
%     \tcp{Training process in one epoch}
%     \For{Iteration i}{
%     \tcp{Update the model to align neuron importance}

%     $\mathcal{L}\leftarrow \mathcal{L_{\tool}}$
    
%     $\theta \leftarrow \theta-\eta \nabla_{\Theta}\mathcal{L}$
%     \\
%     \tcp{Prune less important neurons}
    
%     \If{$i \% pf = 0 \And {\mathcal{L} < pf}$}
%     {
%     \tcp{Sort neurons according to importance}
%     sort()
    
%     \tcp{Remove neurons}
%     prune($ppi, pnm$)
%     }
%     }
%     \end{algorithm}
% \end{minipage}
% \end{wrapfigure}
% \todo{
% A large neural network model could fit extremely well on the training dataset. However, the coverage of the training data is limited compared to the large number of model parameters. The model is prone to memorize all the data points in the training data, which subverts the performance our regularization on the testing data and causes overfitting. }

% \todo{
% In the context of fairness constraints, this is particularly problematic~\cite{overfitting}. Specifically, the fairness constraints are satisfied on the training data while severely violated on test data (\eg, a classifier trained to produce 10\% statistical parity on the training data could show 80\% statistical parity on the test data.) The mainstream methods to stop overfitting include the following: data augmentation, early stopping and so on. These methods are orthogonal to the method \textbf{Neuron Alignment Method}. Compared with early stopping, the pruning method could improve the generalization both on the classification constrasints and the fairness constraints, which further reduces the trade-off.} 
% \textbf{Selective Strategy Based on Pruning.} In a DNN model, there usually exist some neurons that do not contribute positively to the final classification \cite{deeplift}. Aligning such redundant neurons will introduce extra computation cost. More importantly, we hypothesize that the alignment of such neurons that do not contribute positively might "distract" the model from optimizing the alignment of important neurons (supported by the experimental results in \ref{sec:mpa}). An intuitive method to avoid the indiscriminative alignment is to set thresholds to filter important neurons. However, setting thresholds in different phases across multiple layers is too complex. 
% To address such issues, we propose to directly prune the less important neurons in an iterative way according to the aligned neuron importance. 
% In this way, the redundant neurons are removed and the preserved neurons could better characterize the decision rationale, making the alignment of neuron importance more precise. 

% The training process in each epoch is as follows:
% \begin{itemize}[leftmargin=*]
%     \item Training step. Parameters in the trained model are updated by gradient descent with the loss function $\mathcal{L_{\text{\tool}}}$. The model is trained to align the importance of neurons preserved after pruning.
%     \item Pruning step. After a number of minibatches, the less important neurons are selected to be directly pruned according to the aligned neuron importance. 


% \end{itemize}


% Overall, we propose \tool to selectively align neuron importance to achieve \task for better fairness.





==> sections/preliminaries.tex <==
\section{Group Fairness}
% In this paper, we propose to ensure fair decision rationales for different subgroups in the spirit of decomposing DNNs. In this section, we first provide the notations of this paper; we then propose to analyze and characterize the decision rationale of DNNs; finally, we provide our Selective Neuron Importance Alignment approach to mitigate the trade-off.
In this section, we first provide the notations of this paper; we then analyze the larger trade-off; we further introduce our definition to decision rationale discrimination.

%we define fair decision rationale from the perspective of structural pruning. Considering that it is difficult to directly optimize the model to achieve the fair decision rationale, we first characterize the decision rationale for individual subgroup, and then propose a method to align the characterization of decision rationales for different subgroups to achieve fair decision rationale for the model.  Specifically, we propose to estimate the neuron importance of the model to characterize the decision rationale for individual subgroup. On the top of the characterization, we then put forward a method to analyze the divergence of decision rationales between different subgroups. Finally, we propose our method \tool to selectively align the neuron importance to align the decision rationales between different subgroups.

\subsection{Preliminaries}
\label{sec：not}
%
Given a dataset $\mathcal{D}$ with data sample $x \in \mathcal{X}$, label $y \in \mathcal{Y}$ and sensitive attribute $a \in \mathcal{A}$ (\eg, gender, race, age), the deep learning model learns a classification function $\text{F}(\cdot): \mathcal{X} \rightarrow\mathcal{Y}$ with the parameters $\mathbf{W} = \{w_0, w_1, ...\}$.
%
The DNN model $\text{F}(\cdot)$ consists of $L$ layers where the $l$-th layer is represented as $\text{F}_l(\cdot)$ with $ l = 1,...,\mathrm{L}$ and contains a set of neurons. 
%
We name the $m$-th neuron at the $l$-the layer as $w_{m}^{l} \in \text{F}_{l}$.
%
We can split the sample space to subgroups according to a sensitive attribute $a$. For example, with the gender attribute, we have male and female subgroups. 
%
A fair DNN model $\text{F}(\cdot)$ is desired to achieve similar accuracy to get consistent accuracy on the different subgroups (\eg, male and female subgroups).

% The training target following the principle of empirical risk minimization (ERM) is to minimize the error $E$: 
% $\min_\mathbf{W} E(\mathbf{D}, \mathbf{W})$. 
%We refer this training method as \textbf{ERM} (empirical risk minimization).

Following existing works \citep{dp} and \citep{eo}, we use two group metrics, \ie, demographic parity (DP) and equalized odds (EO), to evaluate DNN's fairness.
%
For ease of notation, we introduce them through the binary classification and a binary sensitive attribute.
%
In terms of DP, it evaluates whether different subgroups share the same average of algorithmic decisions, which can be represented as 
%
\begin{align} \label{equa:DP}
\text{DP}(x) = |p(\hat{y}=1 | a=0) - p(\hat{y}=1 | a=1)|,
\end{align}
%
where $p(\hat{y}=1 | a=0)$ and $p(\hat{y}=1 | a=1)$ denote the predictions of $\text{F}(x)$ and mean the probabilities of the input sample to be the category `$\hat{y}=1$' with the attribute to be $a=0$ and $a=1$, respectively. Intuitively, if the $F$ is fair \wrt the attribute `$a$', DP should be zero.
%
EO measures whether different subgroups have the same predicted probability distributions and is defined as
% requiring the outcomes conditioning on $y$. It asserts: $\frac{p( \hat{y}=1 | a=0, y=1)}{ p(\hat{y}=1 | a=1, y=1)} = 1$ and $\frac{p( \hat{y}=1 | a=0, y=0)}{ p(\hat{y}=1 | a=1, y=0)} = 1$ ~\citep{fair_review}.
% Specially, the calculation is defined as:
%
\begin{align} \label{equa:EO}
\text{EO}(x) = \sum_{t \in \{0, 1\}}|{p(\hat{y}=1 | a=0, y=t) - p(\hat{y}=1 | a=1, y=t)}|,
\end{align}
%
where ${p(\hat{y}=1 | a=0, y=t)|t=0,1}$ and ${p(\hat{y}=1 | a=1, y=t)|t=0,1}$ denote the predicted probability distributions with the attribute to be $a=0$ and $a=1$, respectively, and are the outputs of $\text{F}(x)$. If the DNN $\text{F}(\cdot)$ is fair, EO is also desired to be zero.

Although straightforward, the above two objective functions are difficult to be optimized in the training process \citep{Madras2018LearningAF}. Then, Madras et al. propose to relax the DP and EO metrics as follows:
%
%-----------------------
\begin{align} \label{equa:DP}
\Delta \text{DP} = \left| E_{x \sim P_0}\text{F}(x) - E_{x \sim P_1}\text{F}(x)\right|. \\
\end{align}
%-----------------------
%-----------------------
\begin{align}
\label{equa:EO}
\Delta \text{EO} = \sum_{t \in \{0, 1\}}\left| E_{x \sim P_0^t}F(x) - E_{x \sim P_1^t}F(x)\right|.
\end{align}
%-----------------------

where $P$ is the joint distribution of x and y, $P_s = P(\cdot|a=s)$ and $P_s^t = P(\cdot|a=s, y=t), s,t \in \{0,1\}$. 

\textit{Outcome Justice} is to ensure that the decision results (\ie the outputs of DNNs) of different subgroups are equal. A direct way to achieve the decision results fairness is to add regularization of $\Delta DP$ and $\Delta EO$ in the training process. Hereby, the target of optimizing decision results fairness (\textit{Outcome Justice}) could be formulated as:
\begin{equation}
\label{equa:DP}
\min  E_{x \sim P}F(x) + \lambda \Delta DP,  \min  E_{x \sim P}F(x) + \lambda \Delta EO. \\
\end{equation}
In the following sections, we denote this results alignment method as \textbf{ResAlign}. 

\subsection{Analysis of The Fairness Trade-off}
As introduced in~\citet{it}, some fairness metrics like $\Delta DP$ and $\Delta EO$ are incompatible with the ERM training target, incurring trade-offs between fairness and model accuracy. However, as we observed in ~\citet{fairmixup} and ~\citet{Du2021FairnessVR}, training with such fairness metrics suffers from a severer trade-off than expected. Recent studies show that although some similar samples arrive at the same decision results, the neuron behaviors might be disparate. \litl{Check the theory part of such papers. Adversarial examples overfit easily blablabla.} Such work enlightens us to analyze the neuron behaviors behind the fair decision results for understanding the cause of the severer trade-off.

\subsection{Definition of Neuron Discrimination}

% In accordance with \textit{Procedural Justice}, the rationale behind the decisions of the model should also be consistent. 
In our paper, we define the \task in the spirit of decomposing DNNs. 
For a classification task independent of gender difference, we assume the classification should only rely on gender-irrelevant features, which means the decision rationale should be non-discriminatory to any subgroup.
From the perspective of neuron function analysis, if the model still achieves fair decision results after being decomposed to an arbitrary sub-architecture, the decision rationale of the model should be fair. Based on the above analysis, the definition of neuron discrimination can be formulated as :

% We expect that the decision process of the model is fair to different subgroups. We assume that the constraint $\Delta EO$ is satisfied in the training process, \ie, $\Delta EO = 0$. We can get $E_{x \sim P_0^t}F(x, \mathbf{W}) = E_{x \sim P_1^t}F(x, \mathbf{W})$ for $t \in \{0,1\}$. Then we can convert the fair decision process requirement into the constraint that removing each individual neuron could cause same influence to the empirical error of different subgroups. We formulate the influence gap for the $m$-th neuron on the $l$-th layer of model F (under the EO fairness metric) as follows:
% \begin{equation}
% \begin{aligned}
% \label{equa:def}
% \min\sum_l^L\sum_m^{M_l}\mathbf{Gap}_m^{l} &= \min\sum_l^L\sum_m^{M_l}\sum_{t \in \{0, 1\}} |E_{x \sim P_0^t}F(x, \mathbf{W}|w_m^l=0) - E_{x \sim P_1^t}F(x,  \mathbf{W}|w_m^l=0)|^2
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% \label{equa:def}
% \sum_{t \in \{0, 1\}} |E_{x \sim P_0^t}F(x, \mathbf{W}|\bar{\mathbf{W}}=0) - E_{x \sim P_1^t}F(x,  \mathbf{W}|\bar{\mathbf{W}}=0)|^2 = 0.
% \end{aligned}
% \end{equation}

\begin{equation}
\begin{aligned}
\label{equa:def}
\mathbf{Gap_{\bar{\mathbf{W}}}} = |E_{x \sim P_0}F(x, \mathbf{W}|\bar{\mathbf{W}}=0) - E_{x \sim P_1}F(x,  \mathbf{W}|\bar{\mathbf{W}}=0)|^2.
\end{aligned}
\end{equation}

where $\bar{\mathbf{W}}$ is an arbitrary set of neurons to be pruned. 
% Considering that the above formula is difficult to estimate and optimize due to the huge searching space of $\bar{\mathbf{W}}$, 
% In other words, the \task constraint above can be deemed that removing arbitrary neuron should cause the same impacts of the decision process to different subgroups. 

We take a greedy strategy and assume the independence of each neuron, thus we could further estimate the impact of removing a set of neurons $\bar{\mathbf{W}}$ as the accumulation of the impacts of removing each individual neuron in $\bar{\mathbf{W}}$. Thus, we first formulate the impacts gap between different subgroups caused by removing individual neurons as:

% \begin{equation}
% \begin{split}
% \label{equa:def2}
% \mathbf{Gap}_m^{l} = \sum_{t \in \{0, 1\}} &(| (E_{x \sim P_0^t}F(x, \mathbf{W}) - E_{x \sim P_0^t}F(x, \mathbf{W}|w_m^l=0))| ^2 \\ 
% & - |(E_{x \sim P_1^t}F(x, \mathbf{W}) - E_{x \sim P_1^t}F(x, \mathbf{W}|w_m^l=0)) | ^2).
% \end{split}
% \end{equation}

% \begin{equation}
% \begin{split}
% \label{equa:def2}
% \mathbf{Gap}_m^{l} = \sum_{t \in \{0, 1\}} &|( E_{x \sim P_0^t}F(x, \mathbf{W}) - E_{x \sim P_0^t}F(x, \mathbf{W}|w_m^l=0)) ^2 \\ 
% & - (E_{x \sim P_1^t}F(x, \mathbf{W}) - E_{x \sim P_1^t}F(x, \mathbf{W}|w_m^l=0)) ^2|
% \end{split}
% \end{equation}

% \begin{equation}
% \begin{split}
% \label{equa:def2}
% \mathbf{Gap}_m^{l} = &| ( E_{x \sim P_0}F(x, \mathbf{W}) - E_{x \sim P_0}F(x, \mathbf{W}|w_m^l=0)) ^2 \\ 
% & - (E_{x \sim P_1}F(x, \mathbf{W}) - E_{x \sim P_1}F(x, \mathbf{W}|w_m^l=0)) ^2|
% \end{split}
% \end{equation}

\begin{equation}
\begin{aligned}
\label{equa:def2}
\mathbf{Gap_{\bar{\mathbf{W}}}} = \sum_l^L\sum_m^{\bar{\mathbf{W}}_l} \mathbf{Gap}_m^{l} = \sum_l^L\sum_m^{\bar{\mathbf{W}}_l} |E_{x \sim P_0}F(x, \mathbf{W}|w_m^l=0) - E_{x \sim P_1}F(x,  \mathbf{W}|w_m^l=0)|^2.
\end{aligned}
\end{equation}

where $\mathbf{Gap}_m^{l}$ represents the impacts gap caused by removing neuron $m$ on layer $l$, and $\bar{\mathbf{W}}_l$ is the neurons to be pruned on layer $l$.
% The definition of \task could be reformulated as $\sum_l^L\sum_m^{\bar{\mathbf{W}}_l}\mathbf{Gap}_m^{l} = 0$, where  $\bar{\mathbf{W}}_l$ is the neurons to be pruned on layer $l$.
Even so, it is still rather difficult to directly estimate the $\mathbf{Gap}$ value for all neurons and optimize the training target $\min\mathbf{Gap_{\bar{\mathbf{W}}}}$.
